Prompt Tuning with Diffusion for Few-Shot Pre-trained Policy Generalization

Offline reinforcement learning (RL) methods harness previous experiences to derive an optimal policy, forming the foundation for pre-trained large-scale models (PLMs). When encountering tasks not seen before, PLMs often utilize several expert trajectories as prompts to expedite their adaptation to new requirements. Though a range of prompt-tuning methods have been proposed to enhance the quality of prompts, these methods often face optimization restrictions due to prompt initialization, which can significantly constrain the exploration domain and potentially lead to suboptimal solutions. To eliminate the reliance on the initial prompt, we shift our perspective towards the generative model, framing the prompt-tuning process as a form of conditional generative modeling, where prompts are generated from random noise. Our innovation, the Prompt Diffuser, leverages a conditional diffusion model to produce prompts of exceptional quality. Central to our framework is the approach to trajectory reconstruction and the meticulous integration of downstream task guidance during the training phase. Further experimental results underscore the potency of the Prompt Diffuser as a robust and effective tool for the prompt-tuning process, demonstrating strong performance in the meta-RL tasks.

==> sections/2_ReW.tex <==
\vspace{-0.05in}
\section{Related Work}
\vspace{-0.05in}

\subsection{Offline RL as Sequence Modeling}

Offline RL has emerged as a prominent sequence modeling task and Transformer-based decision models have been applied to this domain. 
%
The primary objective is to predict the next sequence of actions by leveraging recent experiences, encompassing state-action-reward triplets.
%
This approach can be effectively trained using supervised learning, making it highly suitable for offline RL and imitation learning scenarios. 
%
Various studies have investigated the utilization of Transformers in RL under the sequence modeling paradigm, including Gato \citep{reed2022generalist}, Multi-Game DT \citep{lee2022multi}, Graph DT \citep{hu2023graph},  and the survey work \citep{hu2022transforming}.
%
In this paper, we propose a novel approach that builds upon the concepts of Prompt-DT \citep{PDT, hu2023prompt} while incorporating prompt-tuning techniques with diffusion models to significantly enhance the model's performance.

\vspace{-0.05in}
\subsection{Diffusion Models in RL}

Diffusion models (DMs) have emerged as a powerful family of deep generative models with applications spanning CV \citep{chen2023hierarchical, liu2023intelligent}, NLP \citep{li2022diffusion, bao2022all}, and more recently, RL \citep{janner2022planning, ajay2022conditional, yu2020meta, ni2023metadiffuser}.
%
In particular, Diffuser \citep{janner2022planning} employs DM as a trajectory generator, effectively showcasing the potential of diffusion models in this domain. 
%
A consequent work \citep{ajay2022conditional} introduces a more flexible approach by taking conditions as inputs to DM. 
%
This enhancement enables the generation of behaviors that satisfy diverse combinations of conditions, encompassing constraints and skills.
%
Furthermore, Diffusion-QL \citep{wang2022diffusion} extends DM to precise policy regularization and injects the Q-learning guidance into the reverse diffusion chain to seek optimal actions.
%
And \citet{pearce2023imitating, reuss2023goal} apply DM in imitation learning to recover policies from the expert or human data without reward labels.
%
Due to its capability to model trajectory distributions effectively, our study utilizes DM for generating prompts using few-shot trajectories, thereby ensuring the precision of generated prompts.

\vspace{-0.05in}
\subsection{Prompt Learning}
Prompt learning is a promising methodology in NLP involving the optimization of a small number of input parameters while keeping the main model architecture unchanged.
%
The core concept of prompt learning revolves around presenting the model with a cloze test-style textual prompt, expecting the model to fill in the corresponding answer.
%
Autoprompt \citep{shin2020autoprompt} proposes an automatic prompt search methodology for efficiently finding optimal prompts, while recent advancements in prompt learning have incorporated trainable continuous embeddings for prompt representation \citep{li2021prefix, lester2021power}.
%
Furthermore, prompt learning techniques have extended beyond NLP and the introduction of continuous prompts into pre-trained vision-language models has demonstrated significant improvements in few-shot visual recognition and generalization performance \citep{zhou2022learning, zhou2022conditional}.
%
In the context of RL, Prompt-tuning DT \citep{hu2023prompt} stands out for introducing prompt-tuning techniques using a gradient-free approach, aiming to retain environment-specific information and cater to specific preferences. 
%
In contrast, our approach leverages DM to directly generate prompts, incorporating flexible conditions during the generation process, which has resulted in notable performance in the target tasks.
